Credit Assignment Techniques in Stochastic Computation Graphs

Stochastic computation graphs (SCGs) provide a formalism to represent structured optimization problems arising in artificial intelligence, including supervised, unsupervised, and reinforcement learning. Previous work has shown that an unbiased estimator of the gradient of the expected loss of SCGs can be derived from a single principle. However, this estimator often has high variance and requires a full model evaluation per data point, making this algorithm costly in large graphs. In this work, we address these problems by generalizing concepts from the reinforcement learning literature. We introduce the concepts of value functions, baselines and critics for arbitrary SCGs, and show how to use them to derive lower-variance gradient estimates from partial model evaluations, paving the way towards general and efficient credit assignment for gradient-based optimization. In doing so, we demonstrate how our results unify recent advances in the probabilistic inference and reinforcement learning literature.

==> Stochastic Computation Graphs - Values and Critics/ext/shared_defs.tex <==
% \usepackage{amsmath}

\newcommand{\dbydy}[1]{\frac{\partial}{\partial #1}}
\newcommand{\dxbydy}[2]{\frac{\partial#1}{\partial #2}}
\newcommand{\dbyd}{\frac{\partial}{\partial \theta}}
\newcommand{\dbydp}{\frac{\partial}{\partial \phi}}

\newcommand{\DbyDy}[1]{\frac{d}{d #1}}
\newcommand{\DxbyDy}[2]{\frac{d #1}{d #2}}
\newcommand{\DbyDt}{\frac{d}{d \theta}}
\newcommand{\DbyDp}{\frac{d}{d \phi}}


\newcommand{\Par}{\operatorname{Par}}
\newcommand{\gIn}{\mathcal{I}}
\newcommand{\gOut}{\mathcal{O}}
\newcommand{\pth}{p_{\theta}}
\newcommand{\Pth}{P_{\theta}}
\newcommand{\pgt}{REINFORCE$_2$}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\rnnup}{h}
\newcommand{\qphi}{q_{\phi}}
\newcommand{\meanparam}{\kappa}
\newcommand{\precd}{\prec^{\scriptscriptstyle D}}
\newcommand{\succd}{\succ^{\scriptscriptstyle D}}
\newcommand{\sg}[1]{\widetilde{#1}}
\newcommand{\hV}{{\hat{V}^\phi}}
\newcommand{\hQ}{{\hat{Q}^\phi}}

\newcommand {\p}[1]{#1^+}
\newcommand{\cInp}{\Theta}
\newcommand{\cX}{\mathcal{X}}

\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\bcI}{\overline{\mathcal{I}}}
\newcommand{\bcB}{\overline{\mathcal{B}}}
\newcommand{\bcC}{\overline{\mathcal{C}}}
\newcommand{\bcR}{\overline{\mathcal{R}}}
\newcommand{\bcF}{\overline{\mathcal{F}}}
\newcommand{\bcD}{\overline{\mathcal{D}}}
\newcommand{\bcL}{\overline{\mathcal{L}}}
\newcommand{\bcX}{\overline{\Theta}}
\newcommand{\bcG}{\overline{\mathcal{G}}}
\newcommand{\bcV}{\overline{\mathcal{V}}}
\newcommand{\bcY}{\overline{\mathcal{Y}}}
\newcommand{\gradph}{\grad_{\phi}}
\newcommand{\simpleheading}[1]{\begin{flushleft}\textbf{#1}\end{flushleft}}
\newcommand{\inp}{\theta}
\newcommand{\outp}{c}
\newcommand{\anc}[1]{\textsc{deps}_{#1}}
\newcommand{\parent}[1]{h({#1})}
\newcommand{\comment}[1]{}
\newcommand{\surr}{L(\cX,\cS)}
\newcommand{\stoch}{\textsc{stoch}}
\newcommand{\determ}{\textsc{determ}}
\newcommand{\stack}[1]{\begin{substack}#1\end{substack}}
\newcommand{\sortnodes}{\textsc{topsort(nodes)}}
\newcommand{\Children}{\operatorname{Children}}
\newcommand{\pe}{\mathrel{+}=}
\newcommand{\nondesc}[1]{\textsc{NonInfluenced}(#1)}
\newcommand{\myint}[1]{\int \! \! #1 \ }
\newcommand{\tiltheta}{\tilth}

\newcommand{\gradth}{\nabla_\theta}
\newcommand{\rp}{\tilde}
\newcommand{\ch}{\check}

\DeclarePairedDelimiter{\lrbrack}{[}{]}
\DeclarePairedDelimiter{\lrbrace}{ \{ }{ \} }
\DeclarePairedDelimiter{\lrparen}{(}{)}

\newcommand{\given}[1][]{\:#1\vert\:}
\newcommand{\dgiven}[1][]{#1\mkern-0.8mu\big\vert}
\newcommand{\bigdgiven}[1][]{#1\mkern-0.8mu\Big\vert}
\newcommand{\suchthat}{\:\vert\:}
\newcommand{\grad}{\nabla}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Ea}[1]{\E\left[#1\right]}
\newcommand{\eqdef}{\overset{\Delta}{=}}
\newcommand{\mb}{\mathbf}
\newcommand{\bx}{\mathbf{x}}

